Positive Lynden-Bell derivative as a ticket to the bar trap?

We have translated the results of $N$-body simulations of one barred model into the language of action variables and frequencies. Using this language, we analysed the behaviour of all orbits in the model on a large time scale at the stage of a mature bar. We show that the orbits join the bar while preserving their adiabatic invariant, which takes into account the 3D structure of the orbits. This allows us to apply the concept of the Lynden-Bell derivative for each of these orbits and trace how the sign of the derivative changes, i.e. how asynchronous changes in angular momentum $L_z$ and orbital precession rate $\Omega_\mathrm{pr}$ (normal orbital mode) change to synchronous (abnormal mode). The transition to the abnormal mode occurs when $\Omega_\mathrm{pr}$ reaches the angular velocity of the pattern $\Omega_\mathrm{p}$, after which the orbit becomes stuck in the bar trap. All this happens against the background of secular changes in actions ($L_z$ decreases, $J_\mathrm{R}$ and $J_z$ increase). At the same time, corotation particles near two stable Lagrange points are also subject to secular changes in their actions. They increase $L_z$ and drift to the periphery, shifting corotation outwards. We also show that a change in the orbital mode from normal to abnormal and the trapping of orbits in a bar is possible only when the bar speed decreases with time, regardless of what is causing the bar to slow down. Our findings clarify and expand the picture of bar formation and evolution in numerical models.

==> pgfgraphicsmacros.tex <==
\usepackage{adjustbox} 
\usepackage{import} 
% i know what i'm doing!
\makeatletter
\def\import@pgf@picture#1\@end{%
  \def\@dir{}\def\@file{}%
  \parse@paths#1/\relax/%
  \expandafter\expandafter\expandafter\import%
  \expandafter\expandafter\expandafter{\expandafter\@dir\expandafter}\expandafter{\@file}%
} % adapted parser by David Carlisle, https://tex.stackexchange.com/a/84804
\def\parse@paths#1/#2/{%
  \edef\@trailing{#2/}%
  \ifx\relax#2\edef\@file{#1}\edef\@trailing{}%
  \else \edef\@dir{\@dir#1/}\expandafter\expandafter\expandafter\parse@paths\expandafter\fi\@trailing%
}
% \def\@import@pgf@picture#1/#2\@end{\import{#1}{#2}}
\newcommand*{\includepgfgraphics}[2][]{%
  \begingroup%
  \ifx &#1&\import@pgf@picture #2\@end%
  \else \begin{adjustbox}{#1}\import@pgf@picture #2\@end\end{adjustbox}%
  \fi\endgroup%
}
\makeatother


==> reviewmacros.tex <==
% setup authorship colors
\RequirePackage{xcolor}
\RequirePackage{etoolbox}

\makeatletter
\newwrite\@todofile
\AtBeginDocument{\immediate\openout\@todofile=todo.txt}
\AtEndDocument{\immediate\closeout\@todofile}
\newcommand*{\todo}[3][]{%
  \begingroup%
  \edef\@isdone{#1}\def\@donestring{done}\def\@doneflag{}%
  \edef\@authors{#2}\def\@task{#3}%<-- not expand this one
  \def\do##1{@##1\space}%
  \def\printauthors{%
    \expandafter\docsvlist\expandafter{\@authors}%
  }%
  \ifdefstrequal{\@isdone}{\@donestring}{%
    \def \@doneflag{x\space}%
    [\textcolor{lightgray}{\texttt{\printauthors \textbf{:} \@task}}]%
  } {[\texttt{\textcolor{red}{\textbf{\printauthors}}\textbf{:} \@task}]}%
  \immediate\write\@todofile{\@doneflag \expandonce{\@task} \space \printauthors}%
  \endgroup%
}
\makeatother


\newcommand*\asc[1]{[{\textcolor{blue}{AS suggests: {#1}}}]}
\newcommand*\ascsc[1]{[{\textcolor{blue}{AS: {#1}}}]}
\let \ascs = \ascsc
%\newcommand*\asen[1]{[{\textcolor{green}{Eng problem: {#1}}}]}
\newcommand*\ascwc[2]{[\textcolor{blue}{#1} {\textcolor{blue}{Suggest: {#2}}}]}
\newcommand*\asen[1]{\textcolor{red}{#1}}
%\newcommand*\asw[1]{[{\textcolor{blue}{AS suggests: {#1}}}]}

% colors
\newcommand{\setnamecolor}[2]{
  \def\do##1{\colorlet{reviewcolors@##1}{#2}}
  \docsvlist{#1}
}
\definecolor{fuchsia}{rgb}{1.0, 0.0, 1.0}
\setnamecolor{Ilia,Iliya,Ilya,IT}{fuchsia!50!black}
\setnamecolor{Anton,AS}{blue}
\setnamecolor{NS}{green}
\setnamecolor{anon}{black}

% #1 = text that is commented
% #1 = author
% #2 = body of comment.
% You may use \c1 \c2 \c3 etc anchors both in the commented text and in the body of the comment.
\newcommand*{\reducedstrut}{\vrule width 0pt height .9\ht\strutbox depth .9\dp\strutbox\relax}
\newcommand*{\commenttextpieces}[3]{%
  \begingroup%
  \setlength{\fboxsep}{0pt}% 
  \def\c##1##2{%
    \ifmmode \let \mathifmathoutside=\ensuremath \else \let\mathifmathoutside=\relax \fi%
    \colorbox{reviewcolors@#2!15}{%
      \reducedstrut%
      \mathifmathoutside{##2}%
      \/%italic correction
      \hbox to 0pt{${}^{\textcolor{reviewcolors@#2}{##1}}$}%
    }}%
  #1%
  \def\c##1{\hbox{${}^{\text{##1}}$}}%
  \thinspace[\textcolor{reviewcolors@#2}{(\textbf{#2}) #3}]%
  \endgroup%
}

\makeatletter
\newcommand*{\startcommenting}[1][]{
  \begingroup
  \let \summary=\commenting@create@summary
  \let \nosummary=\commenting@omit@summary
  \ifblank{#1}%
    {\def\@commenting@author{anon}}
    {\def\@commenting@author{#1}}
  \setlength{\fboxsep}{0pt}% 
  \let \c=\commenting@make@comment
  \let \ins=\commenting@suggest@insert
}
\newcommand*{\commenting@make@comment}[2]{%
  \ifmmode \let \mathifmathoutside=\ensuremath \else \let\mathifmathoutside=\relax \fi%
  \colorbox{reviewcolors@\@commenting@author!15}{%
    \reducedstrut%
    \mathifmathoutside{#2}%
    \/%italic correction
    \hbox to 0pt{${}^{\textcolor{reviewcolors@\@commenting@author}{#1}}$}%
  }}%
\newcommand*{\commenting@suggest@insert}[1]{%
  \textcolor{reviewcolors@\@commenting@author}{#1}%
}
\newcommand{\commenting@annotate@label}[1]{%
  \hbox{${}^{\text{#1}}$}%
}
\newcommand*{\commenting@create@summary}[2][\@commenting@author]{%
  \let \c=\commenting@annotate@label
  \let \ins=\relax
  \thinspace[\textcolor{reviewcolors@#1}{(\textbf{#1}) #2}]%
  \endgroup%
}
\newcommand*{\commenting@omit@summary}{%
  \endgroup%
}
\makeatother


\newcommand*\note[2]{[{\color{reviewcolors@#1}(\textbf{#1})\  #2}]}

